On plethysm conjectures of Stanley and Foulkes: the $2 \times n$ case

We prove Stanley's plethysm conjecture for the $2 \times n$ case, which composed with the work of Black and List provides another proof of Foulkes conjecture for the $2 \times n$ case. We also show that the way Stanley formulated his conjecture, it is false in general, and suggest an alternative formulation.

==> match <==
#FIG 3.2
Landscape
Center
Inches
Letter  
65.00
Single
-2
1200 2
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 4
	 6000 3000 4200 3000 4200 4200 6000 4200
2 2 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 5
	 6000 3000 7200 3000 7200 4200 6000 4200 6000 3000
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 6600 3000 6600 4200
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 3600 6000 3600
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4500 3300 5700 3900
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5100 3300 4500 3900
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5700 3300 5100 3900
2 2 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 5
	 300 3000 3300 3000 3300 4200 300 4200 300 3000
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 300 3600 3300 3600
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3525 3600 3975 3600
2 2 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 5
	 8100 3000 11100 3000 11100 4200 8100 4200 8100 3000
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8700 3000 8700 4200
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9300 3000 9300 4200
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9900 3000 9900 4200
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10500 3000 10500 4200
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 7425 3600 7875 3600
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 3300 8400 3900
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9000 3300 9000 3825
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9600 3300 9600 3825
4 0 0 50 0 1 12 0.0000 2 165 420 4950 4575 $n-k$\001
4 0 0 50 0 1 12 0.0000 2 165 270 6450 4575 $k$\001
4 0 0 50 0 1 12 0.0000 2 165 420 8775 4575 $n-k$\001
4 0 0 50 0 1 12 0.0000 2 165 270 10425 4575 $k$\001
4 0 0 50 0 1 12 0.0000 2 165 405 9375 2775 $\\nu$\001
4 0 0 50 0 1 12 0.0000 2 165 435 6450 2775 $\\nu'$\001
4 0 0 50 0 1 12 0.0000 2 195 1170 1275 2775 $\\mu \\perp \\nu'$\001


==> partial <==
#FIG 3.2
Landscape
Center
Inches
Letter  
65.00
Single
-2
1200 2
2 2 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 1200 1800 4200 1800 4200 3000 1200 3000 1200 1800
2 2 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 6600 1800 9600 1800 9600 3000 6600 3000 6600 1800
2 2 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 1200 3600 4200 3600 4200 4800 1200 4800 1200 3600
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1200 2400 4200 2400
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 7200 1800 7200 3000
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 7800 1800 7800 3000
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 1800 8400 3000
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9000 1800 9000 3000
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1200 4200 4200 4200
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9000 3600 9000 4800
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 4
	 8400 3600 6600 3600 6600 4800 8400 4800
2 2 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 5
	 8400 3600 9600 3600 9600 4800 8400 4800 8400 3600
4 0 0 50 0 1 12 0.0000 2 165 270 1500 2175 $1$\001
4 0 0 50 0 1 12 0.0000 2 165 270 2100 2175 $2$\001
4 0 0 50 0 1 12 0.0000 2 165 270 2700 2175 $3$\001
4 0 0 50 0 1 12 0.0000 2 165 270 3300 2175 $4$\001
4 0 0 50 0 1 12 0.0000 2 165 270 1500 2775 $6$\001
4 0 0 50 0 1 12 0.0000 2 165 270 2100 2775 $7$\001
4 0 0 50 0 1 12 0.0000 2 165 270 2700 2775 $8$\001
4 0 0 50 0 1 12 0.0000 2 165 270 3300 2775 $9$\001
4 0 0 50 0 1 12 0.0000 2 165 360 3900 2775 $10$\001
4 0 0 50 0 1 12 0.0000 2 165 270 6900 2175 $1$\001
4 0 0 50 0 1 12 0.0000 2 165 360 6825 2775 $10$\001
4 0 0 50 0 1 12 0.0000 2 165 270 7500 2175 $7$\001
4 0 0 50 0 1 12 0.0000 2 165 270 7500 2775 $2$\001
4 0 0 50 0 1 12 0.0000 2 165 270 8100 2175 $9$\001
4 0 0 50 0 1 12 0.0000 2 165 270 8100 2775 $4$\001
4 0 0 50 0 1 12 0.0000 2 165 270 8700 2175 $3$\001
4 0 0 50 0 1 12 0.0000 2 165 270 8700 2775 $6$\001
4 0 0 50 0 1 12 0.0000 2 165 270 9300 2175 $5$\001
4 0 0 50 0 1 12 0.0000 2 165 270 9300 2775 $8$\001
4 0 0 50 0 1 12 0.0000 2 165 270 8700 3975 $7$\001
4 0 0 50 0 1 12 0.0000 2 165 270 8700 4575 $2$\001
4 0 0 50 0 1 12 0.0000 2 165 270 9300 3975 $5$\001
4 0 0 50 0 1 12 0.0000 2 165 270 9300 4575 $8$\001
4 0 0 50 0 1 12 0.0000 2 165 270 1425 3975 $1$\001
4 0 0 50 0 1 12 0.0000 2 165 270 2025 3975 $2$\001
4 0 0 50 0 1 12 0.0000 2 165 270 2625 3975 $3$\001
4 0 0 50 0 1 12 0.0000 2 165 270 3300 3975 $4$\001
4 0 0 50 0 1 12 0.0000 2 165 270 3825 3975 $5$\001
4 0 0 50 0 1 12 0.0000 2 165 270 1425 4575 $6$\001
4 0 0 50 0 1 12 0.0000 2 165 270 2025 4575 $7$\001
4 0 0 50 0 1 12 0.0000 2 165 270 2625 4575 $8$\001
4 0 0 50 0 1 12 0.0000 2 165 270 3300 4575 $9$\001
4 0 0 50 0 1 12 0.0000 2 165 360 3825 4575 $10$\001
4 0 0 50 0 1 12 0.0000 2 165 600 600 2475 $\\mu =$\001
4 0 0 50 0 1 12 0.0000 2 165 600 600 4275 $\\mu =$\001
4 0 0 50 0 1 12 0.0000 2 195 555 5025 2475 $\\perp$\001
4 0 0 50 0 1 12 0.0000 2 195 555 5025 4275 $\\perp$\001
4 0 0 50 0 1 12 0.0000 2 165 555 6075 2475 $\\nu =$\001
4 0 0 50 0 1 12 0.0000 2 165 585 6075 4275 $\\nu' =$\001
4 0 0 50 0 1 12 0.0000 2 165 270 3900 2175 $5$\001

